Learning-'N-Flying: A Learning-based, Decentralized Mission Aware UAS Collision Avoidance Scheme

Urban Air Mobility, the scenario where hundreds of manned and Unmanned Aircraft System (UAS) carry out a wide variety of missions (e.g. moving humans and goods within the city), is gaining acceptance as a transportation solution of the future. One of the key requirements for this to happen is safely managing the air traffic in these urban airspaces. Due to the expected density of the airspace, this requires fast autonomous solutions that can be deployed online. We propose Learning-'N-Flying (LNF) a multi-UAS Collision Avoidance (CA) framework. It is decentralized, works on-the-fly and allows autonomous UAS managed by different operators to safely carry out complex missions, represented using Signal Temporal Logic, in a shared airspace. We initially formulate the problem of predictive collision avoidance for two UAS as a mixed-integer linear program, and show that it is intractable to solve online. Instead, we first develop Learning-to-Fly (L2F) by combining: a) learning-based decision-making, and b) decentralized convex optimization-based control. LNF extends L2F to cases where there are more than two UAS on a collision path. Through extensive simulations, we show that our method can run online (computation time in the order of milliseconds), and under certain assumptions has failure rates of less than 1% in the worst-case, improving to near 0% in more relaxed operations. We show the applicability of our scheme to a wide variety of settings through multiple case studies.

==> chapters/appndx/FlyByLogic.tex <==
\section{Fly-by-Logic: Trajectory generation for STL satisfaction}
\label{sec:FbL}

\newcommand{\vl}{\underline{v}}
\newcommand{\vu}{\bar{v}}
\newcommand{\al}{\underline{a}}
\newcommand{\au}{\bar{a}}

Given an STL specification $\formula$ for the mission requirements, we use algorithm \ref{alg:FbL} \cite{pant2018fly} to generate trajectories for the UAS involved in the mission such that they satisfy $\formula$. The algorithm relies on solving an optimization \eqref{eq:HLOptim} to maximize, over these UAS trajectories, the smooth robustness associated with the STL specification. These trajectories, which consist of $N$ jerk-minimizing spline \cite{MuellerTRO15} segments $q^0,\dotsc,q^N$, are parameterized by a set of $N+1$ waypoints (positions in $\mathbb{R}^3$) for each of the $d$ UAS. These waypoints are to be reached sequentially every $dt$ seconds and they form variables for the underlying optimization. This formulation results in trajectories with a total flight time of $T = Ndt$ seconds. Fig. \ref{fig:spline_fig} shows these waypoints, the continuous time spline trajectories $q$ connecting them, and a high-rate ($dt' \ll dt$) discretization $q(kdt')$ of these trajectories for a single UAS. 

The detailed formulation is in \cite{pant2018fly}, the rest of this section gives an overview of the approach and the key results.

\begin{figure}[tb]
\centering
\includegraphics[width=0.48\textwidth]{chapters/appndx/spline_fig}
\vspace{-10pt}
\caption{\small{Planar splines connecting position waypoints $p_0$, $p_1$ and $p_2$. $q^0$ is the continuous spline (positions, velocities and accelerations) connecting $p_0$ and $p_1$ and $q_1$ is the spline from $p_1$ to $p_2$. $q(kdt^{'})$ is the $k^{th}$ sample of $q^0$, with sampled time $dt^{'}$. 
%Note, unlike the stop-go case, non-zero end point velocities mean that the resulting motion is not simply a line connecting the way points.
}}
\label{fig:spline_fig}
\vspace{-5pt}
\end{figure}


 


%\ypcomment{add optimization and the real algorithm with that}
\begin{algorithm}
 \KwData{Specification $\phi$, parameters for optimization $\mathbf{P}_\formula$ \eqref{eq:HLOptim} and initial guess for waypoints $\bar{\mathbf{p}}^d$ of each UAS $d$}
 \KwResult{For each of $d$ UAS, a sequence of $N+1$ waypoints for jerk-minimizing spline generation $\mathbf{p}^1,\dotsc,\mathbf{p}^d $} 
 \While{$0 \leq k \leq N$}{
 At time $t=kdt$: \\	 
 Get current position: ${p}^d_{k},\, \forall d=1,\dotsc,D$ \\
 Set $\bar{\mathbf{p}}_{[0:k]}^d = \mathbf{p}^d_{[0:k]}\, \forall d$ \\ 
 Solve $\mathbf{P}_\formula(\bar{\mathbf{p}}^1,\dotsc,\bar{\mathbf{p}}^D) $ \\ 
 Update $[\mathbf{p}^0,\dotsc,\mathbf{p}^D]$\\
 Give UAS $d$ the next waypoint to track $p^d_{k+1}$, $\forall d$ \\
 Update $\bar{\mathbf{p}}^d = \mathbf{p}^d$ \\	 
 $k \leftarrow k+1$
%  read current\;
%  \eIf{understand}{
%   go to next section\;
%   current section becomes this one\;
%   }{
%   go back to the beginning of current section\;
%  }
 }
 \caption{Fly-by-Logic: Planning for multi-rotor UAS with STL specifications}
 \label{alg:FbL}
\end{algorithm}



\subsection{Waypoint selection for Smooth Robustness maximization }

Let $\mathbf{x} = [\mathbf{p}^0,\dotsc,\mathbf{p}^D] \in \mathbb{R}^{3(N+1)D}$ be the sequence of waypoints (at rate $1/dt$) over all $D$ UAS in the mission and let $\mathbf{q}$ be the associated trajectories discretized at the higher rate $1/dt'$. From the formulation of the jerk-minimizing splines \cite{MuellerTRO15} it was shown in \cite{pant2018fly} that we can compute a linear map $L:\Re^{(T/dt)}\rightarrow \Re^{(T/dt')}$ such that $\mathbf{q} = L(\mathbf{x})$. Also $v^d_{k} \in \mathbb{R}^3$ are the velocities of UAS $d$ at time $kdt$. These are functions of the initial velocity $v^d_0$ and the waypoints $p^d_0,\dotsc,p^d_k$ that the UAS has flown through upto time $kdt$. See the appendix for more details. Finally, the kinematic constraints on the UAS require that its velocity (for every axis of motion) is within the interval $[\vl,\vu]$ and acceleration in $[\al,\au]$. The robustness maximization problem is finally:

\vspace{-10pt}
{\small
	\begin{subequations}
		\label{eq:HLOptim}
		\begin{align}
		&\mathbf{P}_\formula(\bar{\mathbf{p}}^1,\dotsc,\bar{\mathbf{p}}^D): 		
        \max_{\sstraj} \quad \srob_{\formula_s}(L(\mathbf{\sstraj}))\\	
		&\text{s.t. } \forall k=1,\dotsc,N,\, \forall d=1,\dotsc,D \\		
		& \text{LB}_v(v^d_{k-1}) \leq p^d_k- p^d_{k-1} \leq \text{UB}_v(v^d_{k-1}), 
		\label{eq:HL vel constraint}\\
		&\text{LB}_a(v^d_{k-1}) \leq p^d_k-p^d_{k-1} \leq \text{UB}_a(v^d_{k-1}),
		\label{eq:HL acc constraint}	\\
		&\srob_{\formula_s}(L(\sstraj)) \geq \tilde{\epsilon} \label{eq:rholb}
		\end{align}
	\end{subequations}
}

Here, $(\bar{\mathbf{p}}^1,\dotsc,\bar{\mathbf{p}}^D)$ are initial guesses for the waypoints, with the first point for each UAS as their starting positions. Constraints \eqref{eq:HL vel constraint} and \eqref{eq:HL acc constraint} ensure continuous time kinematic feasibility. $\text{LB}_v,\text{UB}_v,\text{LB}_a,\text{UB}_a$ are linear functions of the waypoints that result in the trajectories between them to be kinematically feasible (see Theorem \ref{th:freevelfeas} in the appendix for details).
Constraint \eqref{eq:rholb} ensures that the smooth robustness exceeds a pre-computed lower $\tilde{\epsilon}$ bound such that the resulting trajectories satisfy the STL specification in continuous time (see Corollary \ref{th:strict_srob}). Note that we replace the mission specification $\formula$ with a \textit{strictified} version $\formula_s$ (see section \ref{sec:strictification} for details). The main result regarding the properties of this optimization follows:

\begin{theorem}[Mission satisfaction and kinematic feasibility]
\label{thm:main_opt}
A feasible solution to the optimization \eqref{eq:HLOptim} generates trajectories for the UAS that:
\begin{enumerate}
\item Satisfy the mission specification $\formula$ in continuous time.
\item Are kinematically feasible for the multi-rotor UAS.
\end{enumerate}
\end{theorem}

This theorem is a combination of Theorem \ref{th:freevelfeas} and Corollary \ref{th:strict_srob} in the Appendix which individually prove the two main results here.


\subsection{Numerical issues for large missions}
The initialization $(\bar{\mathbf{p}}^1,\dotsc,\bar{\mathbf{p}}^D)$ is 
crucial, since depending on the initial guesses for waypoints $\bar{\mathbf{p}}^i$, the non-convex optimization of \eqref{eq:HLOptim} might not converge to a trajectory that satisfies the mission specification. One possible way to define $\bar{\mathbf{p}}^i$ such that they equally divide the space between the starting and the goal positions. However, for more complex mission specifications with nested operators (e.g. cycling trajectories where the UAS must loop between two goals), such initialization might lead to infeasible results. Thus, we require a more 
sophisticated way to define $\bar{\mathbf{p}}^i$.

The smoothing constant $C$ used in the definition of smooth
robustness \cite{pant2017smooth} is another important parameter that 
influences the algorithm evaluation. Small $C$ values ($C<30$) lead to a high robustness approximation error, resulting in trajectories that violate given 
mission specifications. On the other hand, large $C$ values ($C>100$) lead to a better smooth robustness approximation, but the algorithm might fail to produce a solution. The latter occurs because smooth approximations of $\min$ and $\max$ operators exceed the largest positive floating-point number (${\approx} 1.8\mathrm{e}{+308}$), thus resulting in an error when evaluating the objective gradient ($\mathtt{NaN}$ is returned). We suggest setting the default value of $C = 30$. Due to the same numerical overflow, the smooth robustness value might reach $\mathtt{Inf}$ for missions with large map sizes (e.g. our urban case study in Section \ref{sec:airportcase}). We avoid this issue by introducing a scaling factor $k$ which scales down map dimensions. Although this reduces the map resolution, it leads to finite robustness values and stable solutions.

\subsection{User interface for mission specification}

The task of writing the STL specification for a given mission requires a level of familiarity with the syntax and grammar of STL, which could result in a barrier towards the widespread use of the FADS framework presented in this paper. In order to mitigate this, we have developed a graphical interface (Fig. \ref{FIG_FbL_GUI}) that allows UAS fleet operators to visually specify and plan upcoming missions. These missions correspond to a fragment of STL \cite{pant2019nasa}, thus allowing our FADS framework to be applied without requiring the end user to be technically familiar with temporal logic and the underlying trajectory planning process.

%\begin{figure}[!htbp]
%	\begin{center}
%		\includegraphics[width= 0.49\textwidth, trim = {13em 0.1em 13em 0}, clip]{FbL_GUIfig_video_MLEdit.pdf}
%	\end{center}
%	\caption{Annotated overview of the Fly-by-Logic graphic user interface (GUI).}
%	\label{FIG_FbL_GUI}
%\end{figure} 

==> chapters/appndx/dynamics.tex <==
\section{UAS dynamics}
\label{sec:dynamics}

\todo{Do we ignore constraints on the
	UAS inputs? The equation~\eqref{eq:dyn_inp}}
\todo{Change xyz axis to capital, but state to just x? Rest of the paper uses x for the state.}

\begin{figure}[h!]
	\centering
	\includegraphics[width=.5\textwidth]{figures/frames.png}
	\caption{Internal world frame with rotation angles $\eta$ (left) and UAS body frame
with angular rates $\omega$ (right). Gravity is denoted as $\mathbf{g}$,
	thrust force $f$ pointing along the axis $e_3$.
		 Figure adapted from \cite{mueller2015computationally}.}
	\label{fig:frames}
\end{figure}

Multi-rotor dynamics have been studied extensively in the
literature \cite{luukkonen2011modelling}, \cite{mueller2015computationally}, and we closely follow the conventions of
\cite{mueller2015computationally}. %Fig. 9 illustrates the following definitions. 

The UAS is modeled as a rigid body with 6
degrees of freedom. The first three are 
the absolute linear position of the UAS in the orthogonal inertial frame, $p = [x, y, z]^\top\in\mathbb{R}^3$. 
The remaining
three are the rotation angles $\eta=[\phi, \theta, \psi]^\top\in\mathbb{R}^3$ that correspond to roll, pitch and yaw, respectfully, of the UAS body
frame with respect to the internal world frame. Rotation at time $t$ is defined by the rotation
matrix $\mathbf{R}\in\mathbb{R}^{3\times3}$, see \cite{luukkonen2011modelling} for the exact expression.
The corresponding time-derivatives of $\eta$ define UAS' angular velocities, $\omega=[\omega_1, \omega_2, \omega_3]^\top$. 

%We write $v = \dot{p}$ for linear velocity and $a 
%=\dot{v}$ for acceleration. 

Let $m$ be the mass of the UAS, $\mathbf{g}=[0,0,-g]^\top$ the acceleration due to gravity and $e_3 = [0, 0, 1]^\top$ a constant vector in the UAS body frame corresponding the thrust force axis\footnote{UAS' thrust direction in the internal world frame is $\mathbf{R}e_3$}, see Figure~\ref{fig:frames}, then
the dynamics is given by
\begin{equation}
\label{eq:dyn}
m\ddot{p} = \mathbf{R}e_3 f + m\mathbf{g}
\end{equation}

\begin{equation}
\label{eq:dyn_inp}
\dot{\mathbf{R}} = \mathbf{R} 
\begin{bmatrix}
0 & -\omega_3 & \omega_2 \\
\omega_3 & 0 & \omega_1\\
-\omega_2 & \omega_1 & 0
\end{bmatrix}
\end{equation}

By substituting matrix $\mathbf{R}$ from \cite{luukkonen2011modelling} in equation~\eqref{eq:dyn}  we obtain the following equation:
\begin{equation}
m\begin{bmatrix}
\ddot{x} \\\ddot{y} \\\ddot{z}
\end{bmatrix}=
\begin{bmatrix}
\cos\psi\sin\theta \cos\phi +\sin\psi\sin\phi \\
\sin\psi\sin\theta\cos\phi - \cos\psi\sin\phi\\
\cos\theta\cos\phi
\end{bmatrix} f - m
\begin{bmatrix}
0 \\ 0\\g
\end{bmatrix}
\end{equation}

With an assumption of no yaw motion (fixed $\psi=0$) we get the following dynamic system: 
\begin{equation}
\label{eq:dyn_simp}
\begin{bmatrix}
\ddot{x} \\\ddot{y} \\\ddot{z}
\end{bmatrix}=
\frac{1}{m}
\begin{bmatrix}
\sin\theta \cos\phi\\
- \sin\phi\\
\cos\theta\cos\phi
\end{bmatrix} f - 
\begin{bmatrix}
0 \\ 0\\g
\end{bmatrix}
\end{equation}

Let the control inputs be roll, pitch and thrust of the UAS, therefore,
$\mathbf{u}=[\phi, \theta, f]^\top\in\mathbb{R}^3$. Denote the full UAS' state as $\mathbf{x}=[x,y,z,\dot{x}, \dot{y},\dot{z}]^\top=[p, v]^\top\in\mathbb{R}^6$. Equation \eqref{eq:dyn_simp} can be written as
\begin{equation}
\label{eq:dyn_general}
\dot{\mathbf{x}} = f(\mathbf{x}, \mathbf{u}).
\end{equation}
The linearization of \eqref{eq:dyn_simp} around hover $\bar{\mathbf{u}}=(0, 0, mg)$ leads to the following system: 
\begin{equation}
\dot{\mathbf{x}} = \left.\frac{\partial f(\mathbf{x}, \mathbf{u})}{d \mathbf{x}}\right\vert_{\substack{\mathbf{x}=\bar{\mathbf{x}}\\ \mathbf{u}=\bar{\mathbf{u}}}} \mathbf{x} +
\left.\frac{\partial f(\mathbf{x}, \mathbf{u})}{d\mathbf{u}}\right\vert_{\substack{\mathbf{x}=\bar{\mathbf{x}}\\ \mathbf{u}=\bar{\mathbf{u}}}} \mathbf{u}
\end{equation}
In other words, we can rewrite \eqref{eq:dyn_general} as the following Linear Time-Invariant (LTI) ODE:
\begin{equation}
\label{eq:dyn_cont}
\dot{\mathbf{x}}(t) = A_c \mathbf{x}(t) + B_c \mathbf{u}(t)
\end{equation}
where 
\begin{equation}
A_c = \left.\frac{\partial f(\mathbf{x}, \mathbf{u})}{d\mathbf{x}}\right\vert_{\substack{\mathbf{x}=\bar{\mathbf{x}}\\ \mathbf{u}=\bar{\mathbf{u}}}} = \begin{bmatrix}
\mathbf{0}_{3\times3} & I_{3\times 3} \\
\mathbf{0}_{3\times3} & \mathbf{0}_{3\times3}
\end{bmatrix},
\end{equation}
\begin{equation}
B_c = \left.\frac{\partial f(\mathbf{x}, \mathbf{u})}{d\mathbf{u}}\right\vert_{\substack{\mathbf{x}=\bar{\mathbf{x}}\\ \mathbf{u}=\bar{\mathbf{u}}}} = \begin{bmatrix}
&\mathbf{0}_{3\times 3}&\\
0 & g & 0\\
-g & 0 & 0 \\
0 & 0 & \frac{1}{m}
\end{bmatrix}.
\end{equation}
Therefore, the UAS dynamics can be described as following: 
\begin{equation}
\label{eq:dyn_simp2}
\begin{bmatrix}
	\ddot{x} \\\ddot{y} \\\ddot{z}
\end{bmatrix}=
\begin{bmatrix}
	g\theta\\
	- g\phi\\
	\frac{1}{m} f
\end{bmatrix} 
\end{equation}
Discretization of equation~\eqref{eq:dyn_cont} following \cite{pant2015co} leads to:
\begin{equation}
\label{eq:dyn_k}
\mathbf{x}_{k+1}= A \mathbf{x}_k + B \mathbf{u}_k.
\end{equation}

The preceding model \eqref{eq:dyn_simp2} is a simplification of complex dynamic interactions.
There exist other more sophisticated UAS models. For example, dynamic model in \cite{bouadi2007nonlinear} includes drag force generated by the air resistance. 
Models studied in \cite{hoffmann2007quadrotor} and \cite{huang2009aerodynamics} include 
dependence of thrust on angle of attack, blade flapping and airflow disruptions.
The influence of aerodynamical effects is complicated
and some of the effects have significant impact
only in high velocities and regimes beyond nominal hover conditions. 
Thus, these effects are excluded from the model used in this paper.
The dynamic model \eqref{eq:dyn_simp2} captures the most relevant dynamics and yields tractable solutions to the trajectory generation problem.
Furthermore, in many applications, for
example, model predictive control, such a simple model is
sufficient, with continuous replanning compensating for modeling inaccuracies.



==> chapters/appndx/dynamics_short.tex <==
\section{UAS dynamics}
\label{sec:dynamics}

%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=.5\textwidth]{figures/frames.png}
%	\caption{Internal world frame with rotation angles $\eta$ (left) and UAS body frame
%with angular rates $\omega$ (right). Gravity is denoted as $\mathbf{g}$,
%	thrust force $f$ pointing along the axis $e_3$.
%		 Figure adapted from \cite{mueller2015computationally}.}
%	\label{fig:frames}
%\end{figure}


The UAS is modeled as a rigid body with 6
degrees of freedom. The first three are 
the absolute linear position of the UAS in the orthogonal inertial frame, $p = [X, Y, Z]^\top\in\mathbb{R}^3$. 
The remaining
three are the rotation angles $\eta=[\phi, \theta, \psi]^\top\in\mathbb{R}^3$ (roll, pitch and yaw) of the UAS body
frame with respect to the internal world frame. 
We assume no yaw motion, i.e. fixed $\psi=0$.
Rotation at time $t$ is defined by the rotation
matrix $\mathbf{R}\in\mathbb{R}^{3\times3}$, see \cite{luukkonen2011modelling} for the exact expression.
The corresponding time-derivatives of $\eta$ define UAS' angular velocities, $\omega=[\omega_1, \omega_2, \omega_3]^\top$. 

%We write $v = \dot{p}$ for linear velocity and $a 
%=\dot{v}$ for acceleration. 

Let $m$ be the mass of the UAS, $\mathbf{g}=[0,0,-g]^\top$ the acceleration due to gravity and $e_3 = [0, 0, 1]^\top$ a constant vector in the UAS body frame corresponding the thrust force axis\footnote{UAS' thrust direction in the internal world frame is $\mathbf{R}e_3$.}. The dynamics is given by:
\begin{equation}
\label{eq:dyn}
m\ddot{p} = \mathbf{R}e_3 f + m\mathbf{g}
\end{equation}

\begin{equation}
\label{eq:dyn_inp}
\dot{\mathbf{R}} = \mathbf{R} 
\begin{bmatrix}
0 & -\omega_3 & \omega_2 \\
\omega_3 & 0 & \omega_1\\
-\omega_2 & \omega_1 & 0
\end{bmatrix}
\end{equation}

%By substituting matrix $\mathbf{R}$ from \cite{luukkonen2011modelling} in equation~\eqref{eq:dyn}  we obtain the following equation:
%\begin{equation}
%m\begin{bmatrix}
%\ddot{x} \\\ddot{y} \\\ddot{z}
%\end{bmatrix}=
%\begin{bmatrix}
%\cos\psi\sin\theta \cos\phi +\sin\psi\sin\phi \\
%\sin\psi\sin\theta\cos\phi - \cos\psi\sin\phi\\
%\cos\theta\cos\phi
%\end{bmatrix} f - m
%\begin{bmatrix}
%0 \\ 0\\g
%\end{bmatrix}
%\end{equation}


%\begin{equation}
%\label{eq:dyn_simp}
%\begin{bmatrix}
%\ddot{x} \\\ddot{y} \\\ddot{z}
%\end{bmatrix}=
%\frac{1}{m}
%\begin{bmatrix}
%\sin\theta \cos\phi\\
%- \sin\phi\\
%\cos\theta\cos\phi
%\end{bmatrix} f - 
%\begin{bmatrix}
%0 \\ 0\\g
%\end{bmatrix}
%\end{equation}

Let the control inputs be roll, pitch and thrust of the UAS, $u=[\phi, \theta, f]^\top\in\mathbb{R}^3$, and let the full state UAS be $x=[X,Y,Z,\dot{X}, \dot{Y},\dot{Z}]^\top=[p, v]^\top\in\mathbb{R}^6$ then the system dynamics can be written as:
\begin{equation}
\label{eq:dyn_general}
\dot{x} = f(x, u).
\end{equation}
Linearization of \eqref{eq:dyn_general} around hover $\bar{u}=(0, 0, mg)$ and
discretization in time following \cite{pant2015co} leads to:
\begin{equation}
\label{eq:dyn_k}
x_{k+1}= A x_k + B u_k.
\end{equation}

%The obtained model \eqref{eq:dyn_k} captures the most relevant dynamics and yields tractable solutions to the trajectory generation problem.

Obtained model \eqref{eq:dyn_k} is a simplification of complex dynamic interactions.
There exist other more sophisticated UAS models. For example, dynamic model in \cite{bouadi2007nonlinear} includes drag force generated by the air resistance. 
Models studied in \cite{hoffmann2007quadrotor} and \cite{huang2009aerodynamics} include 
dependence of thrust on angle of attack, blade flapping and airflow disruptions.
The influence of aerodynamical effects is complicated
and some of the effects have significant impact
only in high velocities and regimes beyond nominal hover conditions. 
Thus, these effects are excluded from the model used in this paper.
The dynamic model \eqref{eq:dyn_k} captures the most relevant dynamics and yields tractable solutions to the trajectory generation problem.




==> chapters/appndx/greedyAlgo.tex <==
\section{Greedy algorithm for conflict resolution}
\label{sec:greedy_alg}

%For a horizon length of $N$ steps, there are $6^{N}$ possible selections for the deconfliction constraints $H^i_k, \, g^i_k$ (6 at each time step in the horizon). 
%%The centralized MILP formulation picks which constraint to use by activating the corresponding binary variable \eqref{eq:CentralMILP}. 
%For CA-MPC, we need a decision making algorithm to pick these constraints as there are no binary variables in the CA-MPC formulations \eqref{eq:drone1mpc}, \eqref{eq:drone2mpc}. 
%
%The following is a greedy approach to this:

Greedy scheme for conflict resolution is formally defined by the Algorithm~\ref{alg:greedy}. For the time steps such that there is no conflict, greedy scheme selects the direction (or side of the hypercube 
\eqref{eq:noconf}) of the most separation between the 
UAS. For the time steps $k$ where there is a conflict, it picks a 
previous maneuver, e.g. decision for a time step $k-1$.

\begin{algorithm}
 \KwData{Pre-planned trajectories: $\mathbf{x_1}, \, \mathbf{x_2}$, a preset maneuver: $\text{preset} \in \{1,\dotsc,6\}$}
 \KwResult{$d_k \in \{1,\dotsc,6\}\, \forall k=\{0,\dotsc, N+1\}$ for conflict resolution maneuvers $H^{d_k},\, g^{d_k}$}
 initialization k=0, \; 
 \While{$k \leq N+1$}{
 \For{$i=\{1,\dotsc,6\}$}
 {$r^{i}_k = g^i - H^i C(x_{1,k}-x_{2,k})$
 }
 %$i[k] = \text{argmax}_i\, (g_i - H_i (x_1[k]-x_2[k]))$ \\
 \eIf{$\exists i|r^i_k \geq 0 $}{
 $d_k = \text{argmax}_i\, r_{i}[k]$
 }
 {$d_k = \text{preset}$
 }
 k = k+1
%  read current\;
%  \eIf{understand}{
%   go to next section\;
%   current section becomes this one\;
%   }{
%   go back to the beginning of current section\;
%  }
 }
 \caption{Greedy conflict resolution}
 \label{alg:greedy}
\end{algorithm}



==> chapters/appndx/rural.tex <==
\section{Case Study: Equipment Surveillance Scenario}
\label{sec:rural_case}

\begin{figure}[tb]
	\begin{center}
		\includegraphics[width=0.7\textwidth]{chapters/appndx/rural_out}
	\end{center}
	{\footnotesize
		\caption{\small Trajectories for 4 UAS tasked with flying over the
			pumpjacks by reaching the all green-colored goal set 
			within 10 minutes, while avoiding the all black-colored 
			obstacles (the
			pumpjacks themselves).}
		\label{fig:rural}}
\end{figure} 


The equipment surveillance scenario taken 
from~\cite{wargo2014unmanned} outlines a low-altitude mission profile 
for four UAS operating within a sparsely populated area. The airspace 
setting is depicted in a Figure~\ref{fig:rural}. This scenario can 
serve as a template
for other rural use cases for UAS such as end-point package
deliveries and wildfire management.

The mission for each UAS $j\in\{1,\ldots,4\}$
is formalized in STL as following:
\begin{equation}
\label{eq:rural_d}
\begin{aligned}
\varphi_j =  \bigwedge_{n=1}^5
\eventually_{[0,10]} (p_j \in \text{Zone}_n)
&\land \eventually_{[9,10]} (p_j \in \text{EndZone}_j) \\
&\land\always_{[0,10]} \neg (p_j \in \text{Unsafe})
\end{aligned}
\end{equation}
where 
$T=10$m is the maximum allowable flight time
allocated to the mission, $\text{Zone}_n$ denotes the airspace region 
directly above each
of the five pumpjacks, $\text{Unsafe}$ denotes the no-fly zones within
the mission environment and $\text{EndZone}_j$ defines the region 
signifying the end of the UAS mission.

Table~\ref{tbl:runtimes_rural} shows the computation times 
for solving the planning problem in a centralized manner versus 
solving for each 
UAS $j$ and its specification $\varphi_j$ separately.



\begin{table}[]
	\renewcommand{\arraystretch}{1.}
	\caption{Computation times for the centralized versus individual 
		UAS planning
	}
	\label{tbl:runtimes_rural}
	
	\centering
	\begin{tabular}{c|c|c|c|c|c|}
		\cline{2-6}
		\multicolumn{1}{l|}{}                   & 
		\textbf{Centralized} & 
		\multicolumn{4}{c|}{\textbf{Independent 
				planning}}                   
		\\ \cline{2-6} 
		& \textbf{4 UAS}    & \textbf{UAS 1} & \textbf{UAS 2} & 
		\textbf{UAS 3} & \textbf{UAS 4} \\ \cline{2-6} 
		\hline\hline
		\multicolumn{1}{|c|}{\textbf{Mean (s)}} & 
		81.918               & 15.596          & 
		17.444            & 
		17.553           &   16.128        \\ \hline
		\multicolumn{1}{|c|}{\textbf{SD (s)}} & 
		27.215           & 6.257        & 
		7.404            & 
		6.912           &  6.764        \\ \hline
	\end{tabular}
\end{table}


==> chapters/appndx/slack_sep.tex <==
\section{Brief discussion on minimum separation and CA-MPC objective value}
\label{sec:slackbad}

\begin{figure}
	\begin{subfigure}[b]{0.4\columnwidth}
		\includegraphics[width=1.25\linewidth]{chapters/appndx/slack_distance153.png}
		%\caption{Picture 1}
		\label{fig:1}
	\end{subfigure}
	\hspace{10pt} %%
	\begin{subfigure}[b]{0.4\columnwidth}
		\includegraphics[width=1.25\linewidth]{chapters/appndx/slack_distance32.png}
		%\caption{Picture 2}
		\label{fig:2}
	\end{subfigure}
\vspace{-10pt}
\caption{\small Slack $\lambda_2$ and minimum separation over time for 
two different 
initial conditions after the random sequence scheme.}
\label{fig:slackbad}
\end{figure}

The condition of Theorem \ref{th:CAMPC_success} could be violated but two UAS could still be separated by more than $\delta$m. This could happen because at the time step $k$ the separation between the two UAS is achieved through some other relative position configurations ($i$ in eq. \ref{eq:pickaside}) compared to the one that is used as a constraint in the optimization. At the time steps $k$ where the robustness tubes of the two UAS are themselves more than $\delta$m apart, having a $\lambda_{2,k}>0$ cannot result in a violation of eq. \ref{eq:msep}. Fig. \ref{fig:slackbad} shows a couple of such examples.

==> chapters/ca_mpc_version2.tex <==
\subsection{Distributed and co-operative collision avoidance MPC}
\label{sec:ca_mpc}

\textbf{CA-MPC optimization for UAS 1:}
Let $\mathbf{x}_1'$ and $\mathbf{u}_1'$ be the optimization variables (new states and inputs) for UAS 1:

\begin{equation}
\label{eq:drone1mpc}
\begin{split}
& \min_{\mathbf{u_1'},\mathbf{\lambda_1}|\mathbf{x_1},\, \mathbf{x_2}} \sum_k \lambda_{1,k} \\
x_{1,0}' &= x_{1,0} \\
x_{1,k+1}' &= Ax_{1,k}' + Bu_{1,k}' \, \forall k=\{0,\dotsc,N\} \\
Cx_{1,k}' &\in P_{1,k} \, \forall k=\{0,\dotsc,N\} \\
H^{d_k} C\,(x_{1,k}'-x_{2,k}) &\leq g^{d_k} + \lambda_{1,k} \forall k=\{0,\dotsc,N+1 \} \\
u_{1,k}' &\in U \forall k=\{0,\dotsc,N \} \\
\lambda_{1,k} &\geq 0 \forall k=\{0,\dotsc,N \}
\end{split}
\end{equation}

This MPC optimization tries to find a trajectory for UAS 1 that minimize the violations $\lambda_{1,k}$ in the minimum separation constraint w.r.t the pre-planned trajectory of UAS 2. The constraints are meant to ensure that UAS 1 respects its dynamics, input constraints, and state constraints imposed by staying inside the robustness tube w.r.t its pre-planned trajectory.
If the objective is $0$, it implies that by UAS 1's maneuvers alone have created separation between the two UASs. If the objective is greater than 0, UAS 1 alone could not create separation and UAS 2 now needs to maneuver as well.

\textbf{CA-MPC optimization for UAS 2:}
In case UAS 1 cannot create minimum separation, UAS 2 now needs to create a new trajectory that does not violate the minimum separation with the new trajectory $\mathbf{x_1'}$ of UAS 1 (w.r.t the same de-confliction constraints $H^{d_k},g^{d_k}$ that UAS 1 tried to satisfy).
%
\begin{equation}
\label{eq:drone2mpc}
\begin{split}
& \min_{\mathbf{u_2'},\mathbf{\lambda_2}|\mathbf{x_1'},\, \mathbf{x_2}} \sum_k \lambda_{2,k} \\
x_{2,0}' &= x_{2,0} \\
x_{2,k+1}' &= Ax_{2,k}' + Bu_{2,k}' \, \forall k=\{0,\dotsc,N\} \\
Cx_{2,k}' &\in {P}_{2,k} \, \forall k=\{0,\dotsc,N\} \\
H^{d_k}C\,(x_{1,k}'-x_{2,k}') &\leq g^{d_k} + \lambda_{2,k} \forall k=\{0,\dotsc,N+1 \} \\
u_{2,k}' &\in U \forall k=\{0,\dotsc,N \} \\
\lambda_{2,k} &\geq 0 \forall k=\{0,\dotsc,N \}
\end{split}
\end{equation}

If the objective here is zero, it means the two UAS have cooperatively created new trajectories that do not conflict. This result, formalized below, is a consequence of the construction of the optimization. We skip the proof for brevity.

\begin{theorem}
\label{th:CAMPC_success}
The feasibility of optimization of \eqref{eq:drone1mpc}, and the existence of optimal solution such that $\sum_k \lambda_{2,k} = 0$ for \eqref{eq:drone2mpc} implies that the resulting two UAS trajectories are non-conflicting and within the robustness tubes of the initial trajectories.
\end{theorem}

\textbf{Note:} this is a conservative result. Indeed, if $\exists k| 
\lambda_{2,k}>0$, it does not necessarily imply that the separation 
requirement of eq. \ref{eq:msep} is violated. A discussion with 
examples is in the Appendix in Section \ref{sec:slackbad}.


Next, the following result captures the relation between the 
existence of a feasible solution for the MILP approach and the 
success of CA-MPC optimizations for the two UAS:

\begin{theorem}
\label{th:MILP_CAMPC_relation}
The non-zero binary variables $b^i_k$ selected by a feasible MILP formulation of eq. \ref{eq:CentralMILP}, when used to select the constraints (defined by $H,\,g$) for the CA-MPC formulations for UAS 1 and 2, imply the existence of: 1) a feasible solution for the optimizations of \eqref{eq:drone1mpc} and 2) a solution for \eqref{eq:drone2mpc} such that $\lambda_{2,k}=0\,\forall k$.  
\end{theorem}

\textit{Proof sketch:} The proof is through construction. Plugging in the $\mathbf{u}'_1$ and $\mathbf{u}'_2$ obtained through the MILP (along with the constraints $H^i_k,\, g^i_k$ selected by the binary variables in the MILP) into eqs. \eqref{eq:drone1mpc} and \eqref{eq:drone2mpc} respectively will result in the constraints of eq. \eqref{eq:drone1mpc} being feasible (with some $\mathbf{\lambda_1} \geq 0$) as well as the constraints of eq. \ref{eq:drone2mpc} being feasible with $\mathbf{\lambda_2} = 0$.

The overall algorithm for Learning-to-Fly is presented in alg. 
\ref{alg:naive}. It is designed be computationally lighter than the 
MILP approach eq. \ref{eq:CentralMILP}, but unlike the MILP it is not 
complete. We show in Section \ref{sec:experiments} through extensive 
simulations that this approach is considerably faster with comparable 
performance.

\begin{algorithm}
	\KwData{Pre-planned trajectories, robustness tubes}
	\KwResult{Sequence of control signals $u_1'$, $u_2'$ for the two UASs}
	\While{Not done}{
		Pick $\text{preset}$ maneuver \\
		Get $\mathbf{d}$ from conflict resolution \\
		UAS 1 solves optimization of \eqref{eq:drone1mpc} \\
		\eIf{$\sum_k \lambda_1[k] == 0$}
		{\textbf{Done}: UAS 1 alone has created separation
		}
		{
			UAS 2 solves optimization of \eqref{eq:drone2mpc} \\
			\eIf{$\sum_k \lambda_2[k] == 0$}{\textbf{Done:} UAS 2 has created 
				separation }
			{\textbf{Not done}: UAS still violate eq. \ref{eq:msep}, try a new maneuver for separation}
		}
		
		Apply control sequences if \textbf{done}, fail if separation is not created.
	} %end while
	\caption{Learning-to-Fly: Decentralized and cooperative collision avoidance for two UAS. Also see fig. \ref{fig:concept}.}
	\label{alg:naive}
\end{algorithm}

==> chapters/priorities.tex <==
\section{UAS Priorities}
\label{sec:priorities}

{\color{red} Here we need to explain how the priorities are defined ($1<2<3<...$) and what they could mean (emergency, preorder, etc)
	For UAS $j<i$, UAS $j$ is trying to de-conflict, \textbf{unless} $i$ also needs to try. 
	Like UAS $i$ will be executing their own trajectories while all UAS $j<i$ are trying to de-conflict with $i$ and all other UAS $k$, $k>j$.}
